A pilot study of the use of LogEx, lessons learned

LogEx is a learning environment that supports students in rewriting propositional logical formulae, using standard equivalences. We organized a pilot study to prepare a large scale evaluation of the learning environment. In this paper we describe this study, together with the outcomes, which teach us valuable lessons for the large scale evaluation.

==> Makefile <==
#-----------------------------------------------------------------------------
# programs

LHS2TEX  := lhs2TeX
PDFLATEX := pdflatex
LATEX    := latex
BIBTEX   := bibtex
GHC      := ghc
SPELL    := ispell
EDITOR   := $(shell if which xemacs > /dev/null 2>&1; then echo xemacs; else echo emacs; fi)
XDVI     := xdvi
GV       := gv
ACRO     := $(shell if test -x /opt/Acrobat7/acroread; then echo /opt/Acrobat7/acroread; else echo acroread; fi)
XPDF     := xpdf
SPELL    := ispellmv
DVIPDFM  := dvipdfm

#-----------------------------------------------------------------------------
# flags

GHCFLAGS     =
LHS2TEXFLAGS = -v --poly -s$(PDFMETHOD)
SPELLFLAGS   = -d british -t -l -p
EDITORFLAGS  =
XDVIFLAGS    = -s 6
GVFLAGS      = -spartan
ACROFLAGS    =
XPDFFLAGS    =
SPELLFLAGS   =  -d british -t -l

#----------------------------------------------------------------------------
# preferences

# supported PDFMETHODs:
# dvipdfm  -> use dvipdfm
# pdftex   -> use pdf(la)tex
# pdflatex -> synonym for pdftex
# none     -> no pdf, produce ps only
PDFMETHOD := pdflatex

# supported FORCEs:
# yes      -> rebuild the TeX file in any case
# no       -> rebuild the TeX file only if changed
FORCE := yes

#-----------------------------------------------------------------------------
# paths

#-----------------------------------------------------------------------------
# project

PROJECT  := pilotlogex
ALLFILES := $(PROJECT).lhs Ideas.bib

-include local.mk

#-----------------------------------------------------------------------------
# initialization

ifeq ($(PDFMETHOD),pdflatex)
PDFMETHOD := pdftex
endif
ifeq ($(FORCE),yes)
FORCETARGET := force
endif

#-----------------------------------------------------------------------------
# rules

ifeq ($(PDFMETHOD),none)
default : ps
else
default : pdf
endif
pdf : $(PROJECT).pdf
ps : postscript
postscript : $(PROJECT).ps

.setup :
	touch .setup

commit : .setup
	svn commit

update : .setup
	svn update

edit :
	$(EDITOR) $(EDITORFLAGS) $(ALLFILES) &

xdvi : $(PROJECT).dvi
	$(XDVI) $(XDVIFLAGS) $(PROJECT).dvi &

gv : $(PROJECT).ps
	$(GV) $(GVFLAGS) $(PROJECT).ps &

acro : $(PROJECT).pdf
	$(ACRO) $(ACROFLAGS) $(PROJECT).pdf &

xpdf : $(PROJECT).pdf
	$(XPDF) $(XPDFFLAGS) $(PROJECT).pdf &

ghci : $(PROJECT).lhs
#	ghci -Wall -fglasgow-exts $(PROJECT).hs
	ghci -v0 -fglasgow-exts -pgmL $(LHS2TEX) -optL--pre $(PROJECT).lhs

spell: $(PROJECT).tex
	egrep -v '$\%' $(PROJECT).tex | $(SPELL) $(SPELLFLAGS) -p $(PROJECT).spell | sort | uniq

spellupdate: $(PROJECT).tex
	egrep -v '$\%' $(PROJECT).tex | $(SPELL) $(SPELLFLAGS) | sort | uniq > $(PROJECT).spell

clean :
	rm -f *~ *% *.aux *.bbl *.blg *.log *.toc *.out
	rm -f $(PROJECT).tex $(PROJECT).[1-9]* *.mpx
	rm .setup

realclean : clean
	rm -f *.dvi *.ps *.pdf

# not very editor friendly
#$(PROJECT).lhs : $(PROJECT).fmt
#	touch $@

%.tex : %.lhs .setup $(FORCETARGET)
	$(LHS2TEX) $(LHS2TEXFLAGS) $< > $@ || rm -f $@

%.hs : %.lhs .setup $(FORCETARGET)
	$(LHS2TEX) --newcode $< > $@ || rm -f $@

%.toc : %.tex
	$(PDFLATEX) $<
	echo "***" > $(<:.tex=.explain)
	grep "Warning.*Rerun" $(<:.tex=.log) >> $(<:.tex=.explain) || true
	touch $@

%.dvi-toc : %.tex
	$(LATEX) $<
	echo "***" > $(<:.tex=.explain)
	grep "Warning.*Rerun" $(<:.tex=.log) >> $(<:.tex=.explain) || true
	touch $@

ifeq ($(PDFMETHOD),pdftex)

%.pdf : %.tex .setup
	sh -c ' \
	  $(PDFLATEX) $<; \
	  if grep -s "Warning: Citation .* undefined" $(<:.tex=.log); \
	    then BIBINPUTS="$(BIB)" $(BIBTEX) $(<:.tex=); $(PDFLATEX) $(<); fi; \
	  while grep -s "Warning.*Rerun" $(<:.tex=.log); \
	    do $(PDFLATEX) $<; done;'

endif

ifeq ($(PDFMETHOD),dvipdfm)

%.pdf : %.dvi
	dvipdfm $<

endif

%.ps : %.dvi
	dvips -o $@ $<

%.dvi : %.tex .setup
	sh -c ' \
	  $(LATEX) $<; \
	  if grep -s "Warning: Citation .* undefined" $(<:.tex=.log); \
	    then BIBINPUTS="$(BIB)" $(BIBTEX) $(<:.tex=); $(LATEX) $(<); fi; \
	  while grep -s "Warning.*Rerun" $(<:.tex=.log); \
	    do $(LATEX) $<; done;'

.SUFFIXES :

.SECONDARY :

.PHONY : force edit xdvi gv acro xpdf spell spellupdate clean realclean commit

force : .setup
	@:

%.pdf : %.ps
	pstopdf $<

%.ps : %.dot.txt
	dot -Tps $< -o $@

